Synthesis of Mathematical programs from Natural Language Specifications

Several decision problems that are encountered in various business domains can be modeled as mathematical programs, i.e. optimization problems. The process of conducting such modeling often requires the involvement of experts trained in operations research and advanced algorithms. Surprisingly, despite the significant advances in the methods for program and code synthesis, AutoML, learning to optimize etc., there has been little or no attention paid to automating the task of synthesizing mathematical programs. We imagine a scenario where the specifications for modeling, i.e. the objective and constraints are expressed in an unstructured form in natural language (NL) and the mathematical program has to be synthesized from such an NL specification. In this work we evaluate the efficacy of employing CodeT5 with data augmentation and post-processing of beams. We utilize GPT-3 with back translation for generation of synthetic examples. Further we apply rules of linear programming to score beams and correct beams based on common error patterns. We observe that with these enhancements CodeT5 base gives an execution accuracy of 0.73 which is significantly better than zero-shot execution accuracy of 0.41 by ChatGPT and 0.36 by Codex.

==> references.tex <==
\begin{thebibliography}
\bibliography{citations}
\bibitem{Mirjalili_2020}Mirjalili, S. \& Mirjalili, S. Special issue on "real-world optimization problems and meta-heuristics".. {\em Neural Computing And Applications}. (2020)
\bibitem{Sierksma_2015}Sierksma, G., Sierksma, G., Zwols, Y. \& Zwols, Y. Linear and integer optimization: Theory and practice. {\em Null}. (2015)
\bibitem{Elizarov_2014}Elizarov, A., Kirillovich, A., Lipachev, E., Nevzorova, O., Solovyev, V. \& Zhiltsov, N. Mathematical knowledge representation: semantic models and formalisms. {\em Lobachevskii Journal Of Mathematics}. (2014)
\bibitem{Parmentier_2021}Parmentier, A. Learning structured approximations of operations research problems. {\em ArXiv}. (2021)
\bibitem{Legat_2021}Legat, B., Dowson, O., Garcia, J. \& Lubin, M. MathOptInterface: A Data Structure for Mathematical Optimization Problems. {\em Informs Journal On Computing}. (2021)
\bibitem{Ofoghi_2020}Ofoghi, B., Mak, V. \& Yearwood, J. A Knowledge Representation Approach to Automated Mathematical Modelling.. {\em ArXiv: Artificial Intelligence}. (2020)
\bibitem{Lippi_2016}Zeynep Kiziltan and Marco Lippi and Paolo Torroni, Constraint Detection in Natural Language Problem Descriptions. {\em ACM}. (2016)
\bibitem{Do_2007}Do, C. Convex Optimization Overview (cnt’d). {\em Null}. (2007)
\bibitem{Pardalos_1999}Pardalos, P. \& Hentenryck, P. The OPL optimization programming language. {\em Null}. (1999)
\bibitem{Rindranirina_2022}
Ramamonjison, R., Li, H., Yu, T., He, S., Rengan, V., Banitalebi-Dehkordi, A., Zhou, Z. \& Zhang, Y. Augmenting Operations Research with Auto-Formulation of Optimization Models from Problem Descriptions. {\em ArXiv}. (2022)
\bibitem{Cambazard_2021}
Cambazard, H., Catusse, N., Brauner, N. \& Lemaire, P. Teaching OR: automatic evaluation for linear programming modelling. {\em A Quarterly Journal Of Operations Research}. (2021)
\bibitem{DAmbrosio_2020}
D’Ambrosio, C., Frangioni, A., Iommazzo, G. \& Liberti, L. A learning-based mathematical programming formulation for the automatic configuration of optimization solvers. {\em Lecture Notes In Computer Science}. (2020)
\bibitem{Yara_2022}
Rizk, Y., Venkateswaran, P., Isahagian, V. \& Muthusamy, V. A Case for Business Process-Specific Foundation Models. {\em Cornell University - ArXiv}. (2022)
\bibitem{codex}
Mark Chen ,Evaluating Large Language Models Trained on Code {\em OpenAI - Arxiv}. (2021)
\bibitem{neeraj_2022}
Neeraj Gangwar, Nickvash Kani. Highlighting Named Entities in Input for Auto-Formulation of Optimization Problems {\em University of Illinois Urbana-Champaign, IL, USA} (2022)
\bibitem{chen_2021}
Evaluating Large Language Models Trained on Code {\em Arxiv} (2021)
\bibitem{hokamp_2017}
Lexically Constrained Decoding for Sequence Generation Using Grid Beam Search {\em https://aclanthology.org/P17-1141} (Hokamp I\& Liu, ACL 2017)
\end{thebibliography}

